Generalizing through Forgetting -- Domain Generalization for Symptom Event Extraction in Clinical Notes

Symptom information is primarily documented in free-text clinical notes and is not directly accessible for downstream applications. To address this challenge, information extraction approaches that can handle clinical language variation across different institutions and specialties are needed. In this paper, we present domain generalization for symptom extraction using pretraining and fine-tuning data that differs from the target domain in terms of institution and/or specialty and patient population. We extract symptom events using a transformer-based joint entity and relation extraction method. To reduce reliance on domain-specific features, we propose a domain generalization method that dynamically masks frequent symptoms words in the source domain. Additionally, we pretrain the transformer language model (LM) on task-related unlabeled texts for better representation. Our experiments indicate that masking and adaptive pretraining methods can significantly improve performance when the source domain is more distant from the target domain.

==> abstract.tex <==
\noindent{\bf Abstract}

\textit{
Risk prediction for hospital mortality detection is important to make life-saving decisions about the critically ill patients in intensive care units (ICU). Several machine learning methods trained on electronic medical records (EMR) have been proposed to address this need. In this paper, we proposed a method to predict in-hospital mortality by taking advantage of clinical time series and radiology reports collected during the first 24 hours of ICU admit time. We used a BERT-based extractor for extracting clinical findings from radiology reports.
It was found that the proposed method increased the model's F1 significantly.
We analyzed the predictions and found the clinical findings' impact could be characterized by two factors -- the number of words in the clinical findings and the occurrences of key medical terms (e.g. pleural, effusion).
The inclusion of the clinical findings increased the precision;
nevertheless, overemphasizing word counts and keywords also made the model hesitate to make positive predictions, which resulted in a decrease of recall.
}

==> figure/algo_mask.tex <==


\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.3]{figure/image/algo_mask.png}
    \caption{Dynamic masking method on frequent phrases from the source domain}
    \label{figure:algo_mask}
\end{figure}






==> figure/analysis_fp_fn.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.6]{figure/image/none_fn_fp.png}
    \caption{False Negatives, Red: wo/ masking, Blue: w/ masking}
    \label{figure:analyse_fn}
\end{figure}


% \begin{figure}[h!]
%     \centering
%     \includegraphics[scale=0.5]{figure/image/none_fp.png}
%     \caption{False Positives, Red: wo/ masking, Blue: w/ masking}
%     \label{figure:analyse_fp}
% \end{figure}



==> figure/finding_example.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.8]{image/finding_example.png}
    \caption{Finding example}
    \label{figure:finding_example}
\end{figure}






==> figure/radiology_report_example.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[scale=0.5]{image/radiology_report_example.png}
    \caption{Radiology report example}
    \label{figure:radiology_report_example}
\end{figure}





==> figure/three_model.tex <==
\begin{figure}[h!]
    \centering
    \includegraphics[width=\textwidth]{image/three_model.png}
    \caption{Models}
    \label{figure:three_model}
\end{figure}






==> section/data.tex <==


\section*{Datasets  (after proofreading)} 
%\label{section:data}
In our experiments, we use the following four datasets. 

The COVID-19 Annotated Text Corpus (CATC) contains clinical notes of 230,000 ambulatory clinic patients treated at UWM between May and June 2020\cite{Lybarger2021ExtractingCD}. CACT contains telephone encounter notes, progress notes, and emergency department notes. 


%COVID-19 Annotated Text Corpus (CATC): The CATC was built from clinical notes of 230,000 ambulatory clinic patients who received treatment at the University of Washington Medical Center (UWM) between May-June 2020\cite{Lybarger2021ExtractingCD}. The CACT contains telephone encounter notes, progress notes of all kinds, and emergency department notes. 

The Lung Cancer Annotated Text Corpus (LATC) was constructed from clinical notes of 4,673 lung cancer patients diagnosed at UWM and Seattle Cancer Care Alliance (SCCA) between 2012 and 2020. LATC includes outpatient progress notes, admission notes, emergency department notes, and discharge notes that were created 24 months prior to cancer diagnosis. 
%Lung Cancer Annotated Text Corpus (LATC): The LATC was built from clinical notes of 4,673 lung cancer patients who were diagnosed with lung cancer at UWM and Seattle Cancer Care Alliance (SCCA) between 2012-2020. LATC includes outpatient progress notes, admission notes, emergency, and discharge notes that were created 24 months prior to cancer diagnosis.  

The Ovarian Cancer Annotated Text Corpus (OATC) is based on the clinical notes of 173 ovarian cancer patients diagnosed at UWM and SCCA between 2012-2021. OATC includes outpatient progress notes, admission notes, emergency department notes, discharge notes, and gynecology notes created 12 months prior to cancer diagnosis.

%Ovarian Cancer Annotated Text Corpus (OATC): The OATC was built from clinical notes 173 ovarian cancer patients who were diagnosed at UWM and SCCA between 2012-2021. OATC included outpatient progress notes, admission, emergency, discharge, and gynecology notes that were created 12 months prior to cancer diagnisis.


The Post-Cancer Diagnosis Annotated Text (PCAT) was built using clinical notes from 2,968 prostate cancer patients and 1,222 Diffuse Large B cell lymphoma patients diagnosed between 2007-2021 at UWM and SCCA. The PCAT contains notes after cancer diagnosis, including notes from urology, oncology, hematology, surgery, radiation oncology, and palliative care.  


%Post-Cancer Diagnosis Annotated Text (PCAT): The PCAT was built from clinical notes of 2,968 prostate cancer patients and 1,222 Diffuse Large B cell Lymphoma patients diagnosed at UWM and SCCA between 2007-2021. PCAT contains notes after cancer diganosis including urology, oncology, hematology, surgery, radiation oncology, and palliative care notes.  

For simplicity, we refer to CATC as \textit{COVID}, LATC as \textit{Lung}, OATC as \textit{Ovarian} and PCAT as \textit{Post}. All these four resources include a variety of clinical notes from UWM. Lung, Ovarian and Post datasets are all related to cancer patients. Lung and Ovarian share the same group of annotators. COVID has more labeled examples. For each domain, we retrieved unlabeled clinical notes from the same distribution as the labeled ones. More details about the data size and inter annotator agreement are summarized in Table \ref{table:stats_data}.
\input{table/stats_data}


%










%\{annoatater aggrement!\}

In this study, we choose Post as the target domain, and we use two sources: one is COVID, and the other is Lung \& Ovarian. We merged Lung and Ovarian because they are relatively small in size. The main differences between source domains and target domains are the diagnosis stages and diseases types of patients. Unlike the target domain, the source domains are not collected for  post-diagnostic stages, and not for prostate or lymphoma cancers. In order to measure the discrepancy between the domains of source and target, we plot the coverage of frequent triggers over both domains in Figure \ref{figure:domain_discrepancy_coverage}. The distribution of triggers in Lung \& Ovarian domain is more similar to the target domain than the COVID source domain. It could be because Lung, Ovarian, and Post are for cancer patients, but COVID is not. 


% \subsection*{Dataset Analysis}


 %Covid is a richer resource, while lung only has annotations on about 200 notes. \ref{table:stats_data}, table-test-size-by-entity, need to see entity types) The distribution of symptom phrases varies across domains. \ref{Table-frequent-syptoms-example} summarizes the frequent symptoms in each domain, and \ref{figure-frequent-syptoms-dist-overlap} shows the overlap of trigger phrases and trigger contexts between the source and the target. Covid is more distant to post compared with lung, one potential reason is lung and post are all from cancer patients. Compared to sources, post-diagnosis notes contain more symptoms specific to hospitalized patients, such as (???).  


\input{figure/analysis_domain_discrepancy} 


==> section/result.tex <==
\section*{Results \& Analysis (after proofreading)}
\subsection*{Baseline}

% \input{table/main_results.tex}

\input{table/results_all_arguments_all} 

Table \ref{table:results_all_arguments_all} summarizes the cross domain results on the trigger and argument extraction. The Lung \& Ovarian source domain performs better than the COVID domain. The human annotator agreement on triggers is 80-83, the trigger F1 is 77.2 for COVID source, and is 79.2 and for Lung / & Ovarian source. 

\subsection*{Effect of Adaptive Pretraining}

Adaptive pretraining improves performance on trigger, \textit{Assertion} and \textit{Characteristics} significantly for the COVID source model. For the models trained on the Lung \& Ovarian source, adaptive pretraining significantly helps \textit{Anatomy} and \textit{Frequency} arguments, but doesn't significantly improve trigger detection.
%Other arguments has lower counts of labels, therefore less persuasive for significance tests.

%78.56 covid_covid_epoch_10_pretrain_allfour_pf1_pte30_lm_seed0_originalVScovid_verify_seed0_original
%78.22.covid_covid_epoch_10_pretrain_allfour_pf1_pte10_lm_seed0_original_pf0VScovid_verify_seed0_original 
%79.00 (0.81, p 0.4189166912940461) %covid_covid_epoch_10_pretrain_allfour_pf1_pte20_lm_seed0_original_pf0 
We pretrain LM on the target domain unlabeled texts along with all source domains texts, its trigger performance on COVID source is 78.6. To our surprise, adding target domain texts to the pretraining corpus of all sources doesn't show further gains. 
We speculate that given source domains are similar to the target, adding target domain texts doesn't greatly improve representation on the target domain data.
%, meanwhile it could dilute the content of Covid domain texts in pretraining, to make the LM less representative for the Covid source. For further discussion, we refer adaptive pretraining only for using the all sources.
%(table-DAPT-dev) shows how we select the epoch numbers based on the validation set results. 

% In order to exclude the unknown effect of prepending domain-specific tokens, we also train on labeled data without the source domain prefix, and we find that including target texts helps lung to post more, but still harms covid to post.
\subsection*{Dynamic Masking Effect}

\input{table/results_infrequent_bin}
%\input{table/results_infrequent_all}

% covid help. 
% removing frequent phrases from the test
% the improvement comes from FN
% check Lung Ovarian pretrain
%Table ~\ref{table:results_infrequent_all} presents the effect of dynamic masking for trigger extraction. 
Masking significantly improves trigger extraction of COVID source models under both pretraining versions, but not the Lung \& Ovarian ones.  It is worth noting masking can bring even extra gains on top of adaptive pretraining benefits for the COVID source.  


We summarize trigger extraction results on truncated test sets to investigate how masking helps extract triggers that are underrepresented in the source (Table \ref{table:results_infrequent_bin}). The gains from masking on COVID source become larger after truncating the test set. For the Lung \& Ovarian source, masking still doesn't significantly improve the results.

%\input{figure/analysis_fp_fn}
% what to present f/p/r
% covid after adaptive pretraiing, masking p from () to (), r from () to ().



We analyze recall and precision changes after masking. An increase in recall is responsible for the improvement in trigger F1 scores when training on the COVID source. After masking, we observe a trade off between higher recall and lower precision for the COVID source models, but recall dominates the change. Contrary to this, the recall and precision scores from the Lung \& Ovarian source are both reduced.
% why inconsistent
% 1. domain discrepency
% 2. FN is due to negative context. Covid has more phrases above the diagonoal.
%\input{figure/analysis_domain_discrepancy}

The inconsistent masking effects on two sources could be explained by the differences in source-target domain discrepancy, and trigger context shifts. 


\textbf{Masking benefits the more distant source domain from the target.} Compared to Lung and Ovarian, COVID is more distantly related to the target. Lung, Ovarian and the target are all for cancer patients, but COVID is not. %Lung \& Ovarian also shares the same annotators with the target domain, but Covid data does not.
Moreover, for the COVID source, symptom distribution shifts more from the source to the target. In Figure \ref{figure:domain_discrepancy_coverage}, the coverages of phrases over the source and target domains overlap more in the Lung & Ovarian source than those in COVID.  

 \textbf{Masking benefits phrases that are are more likely associated with negative contexts in the source than in the target}. The model could take a trigger phrase frequently annotated as non-triggers as a hint for the negative entity type instead of considering the contexts are negative.
To study how triggers' negative context shifts affect masking, we plot positive class ratio of trigger phrases on both source and target domains, which is the likelihood of the phrases annotated as triggers (Figure \ref{figure:analysis_ner_r}). We size and color each point according to the absolute value and sign of the false negative change. We show only false negatives because the trigger detection improvement after masking is due to the reduced false negatives. Most phrases with reduced false negatives are above the diagonal, in other words, the phrases improved after masking are more likely to be annotated as non-triggers in the source domain than in the target. The COVID source has more trigger phrases overly associated with negative contexts and sitting above the diagonal, which leaves the masking method more potential to be effective.
%qualitative table

\input{figure/analysis_neg_r}

% Table~\ref{table:model_compare}.





% \input{table/results_all_arguments_covid}
% \input{table/results_all_arguments_lungovarian} 




==> table/breakdown_prediction_case.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[!ht]
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{|l|ccc|ccc|}
        \hline
        &
        \multicolumn{3}{c|}{positive} &
        \multicolumn{3}{c|}{negative} \\ \cline{2-7}
        &
        \multicolumn{1}{c|}{target} &
        \multicolumn{1}{c|}{+findings} &
        time series &
        \multicolumn{1}{c|}{target} &
        \multicolumn{1}{c|}{+findings} &
        time series \\ \hline
        number of   patients &
        \multicolumn{1}{c|}{1767} &
        \multicolumn{1}{c|}{3031} &
        4409 &
        \multicolumn{1}{c|}{17606} &
        \multicolumn{1}{c|}{16342} &
        14964 \\ \hline
    \end{tabular}
    }
    \caption{Comparison of the number of the positive and negatives predictions made by models with and without the extracted findings.}
    \label{table:breakdown_prediction_case}
\end{table}

==> table/breakdown_word_occurrence.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[!ht]
    \centering
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{|l|ccc|ccc|}
        \hline
        & \multicolumn{3}{c|}{positive}                                   & \multicolumn{3}{c|}{negative}                                \\ \cline{2-7}
        & \multicolumn{1}{c|}{target} & \multicolumn{1}{c|}{+findings} & time series & \multicolumn{1}{c|}{target} & \multicolumn{1}{c|}{+findings} & time series \\ \hline
        present      & \multicolumn{1}{c|}{13.22} & \multicolumn{1}{c|}{15.01} & 11.17 & \multicolumn{1}{c|}{8.43} & \multicolumn{1}{c|}{7.72} & 8.18 \\ \hline
        absent       & \multicolumn{1}{c|}{3.37}  & \multicolumn{1}{c|}{4.25}  & 3.32  & \multicolumn{1}{c|}{3.05} & \multicolumn{1}{c|}{2.86} & 3.01 \\ \hline
        possible     & \multicolumn{1}{c|}{2}     & \multicolumn{1}{c|}{2.25}   & 1.7  & \multicolumn{1}{c|}{1.22} & \multicolumn{1}{c|}{1.12} & 1.17 \\ \hline
        effusion     & \multicolumn{1}{c|}{1.15}  & \multicolumn{1}{c|}{1.26}  & 1.03  & \multicolumn{1}{c|}{0.77} & \multicolumn{1}{c|}{0.72} & 0.74 \\ \hline
        pleural      & \multicolumn{1}{c|}{0.97}  & \multicolumn{1}{c|}{1.08}  & 0.89  & \multicolumn{1}{c|}{0.66} & \multicolumn{1}{c|}{0.62} & 0.63 \\ \hline
        pneumothorax & \multicolumn{1}{c|}{0.55}  & \multicolumn{1}{c|}{0.66}  & 0.59  & \multicolumn{1}{c|}{0.53} & \multicolumn{1}{c|}{0.51} & 0.51 \\ \hline
    \end{tabular}
    }
    \caption{Comparing patients classified by models with and without extracted findings. The average number of keyword occurrences for a patient's extracted findings was shown. Patients were broken down by positives and negatives.}
    \label{table:breakdown_word_occurance}
\end{table}

==> table/main_results.tex <==

% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}
% \usepackage[normalem]{ulem}
% \useunder{\uline}{\ul}{}
\begin{table}[!ht]
    \centering
\begin{tabular}{|l|l|l|l}
\hline
         & lung         & covid         & post \\
         \hline
Bio-Clinical BERT    & 78.9 (0.3)   & 77.2 (0.5)    & xx   \\
+ Dynamic Masking                         & 78.3 (0.8)   & 78.3 (0.7) * & --   \\
         \hline
DAPT (target-relevant)            & 79.5 (0.5)  & 78.6 (0.8)   & xx   \\

+ Dynamic Masking                           & 79.4 (0.5)   & 79.3 (1.0)    & --   \\
         \hline
DAPT (target-relevant + target) & 79.5 (0.3)   & 78.2 (0.9)     & xx  \\
         \hline

\end{tabular}


\caption{This table shows cross-domain transfer results from different sources under the initialization of different pretraining LMs with or without dynamic masking.  We report the average (standard deviation) of five runs with different random seeds for event trigger f1. We run a two-sided t-test to compare results with and without dynamic masking, and use (*) to indicate a p-value below 0.05 and (**) to indicate a p-value below 0.01.
}
    \label{table:main_results}

\end{table}

==> table/mask_code.tex <==
% \SetKwComment{Comment}{/* }{ */}
\RestyleAlgo{ruled} i
\SetKwComment{Comment}{/* }{ */}

\begin{algorithm}
\caption{Masking frequent source domain tokens}\label{alg:mask}
\KwData{$D_{source} = \{(x,y_{e}, y_{r})\}$ 
\Comment*[r]{source domain labeled data} }
\KwResult{$\tilde{D}_{source}$ \Comment*[r]{masked sourc domain labeled data} } 

$MaskList(D_{source}) \gets $   frequent single-token phrases from $D_{source}$\;
\For{$x, y_{e}, y_{r} \in D_{source}$}{\For{token $t \in x$}{
  \eIf{token $t \in  MaskList(D_{source})$ \Comment*[r]{if the token belongs to the mask list}}{
  $m \sim Bernoulli(p_{mask})$ \; 
  \eIf{$m = 1$ \Comment*[r]{apply randomly mask}}{token $t \gets [MASK] $ }  
}
}}
\end{algorithm}
 

==> table/results_all_arguments_covid.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[!ht]
    \centering

\begin{tabular}{lrllll}
\toprule
{} &    NT & Covid &     w/ masking & + Adapt. Pretraining &      w/ masking \\
entity          &       &       &                &                      &                 \\
\midrule
SSx             &  5629 &  77.2 &         78.5** &                 78.6 &  \textbf{79.9*} \\
Assertion       &  5629 &  72.2 &          73.1* &                 74.0 &   \textbf{74.9} \\
Change          &   401 &  55.7 &  \textbf{56.9} &        \textbf{56.9} &   \textbf{56.9} \\
Severity        &   291 &  30.7 &           30.4 &                 29.6 &  \textbf{33.3*} \\
Anatomy         &  3007 &  55.3 &           56.7 &                 57.2 &   \textbf{59.4} \\
Characteristics &  1250 &  22.5 &           22.8 &        \textbf{26.8} &            25.8 \\
Duration        &   837 &  46.5 &           44.1 &                 46.3 &   \textbf{48.4} \\
Frequency       &   301 &  45.9 &           45.6 &                 44.9 &   \textbf{46.6} \\
\bottomrule
\end{tabular}
    \caption{all argument results for the Covid source}
    \label{table:results_all_arguments_covid}
\end{table}


==> table/results_all_arguments_lungovarian.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[!ht]
    \centering

\begin{tabular}{lrllll}
\toprule
{} &    NT & Lung \& Ovarian & w/ masking & + Adapt. Pretraining &     w/ masking \\
entity          &       &                &            &                      &                \\
\midrule
SSx             &  5629 &           79.2 &     78.2** &        \textbf{79.3} &           79.1 \\
Assertion       &  5629 &  \textbf{75.1} &      74.4* &                 75.0 &  \textbf{75.1} \\
Change          &   401 &           47.2 &       44.8 &                 46.1 &  \textbf{47.3} \\
Severity        &   291 &           40.7 &     36.4** &        \textbf{42.2} &           38.5 \\
Anatomy         &  3007 &           60.7 &     58.5** &        \textbf{63.2} &           61.4 \\
Characteristics &  1250 &           15.1 &       16.6 &                 16.3 &  \textbf{17.7} \\
Duration        &   837 &           29.9 &       32.5 &                 30.4 &  \textbf{34.2} \\
Frequency       &   301 &           24.7 &       24.9 &        \textbf{27.3} &           26.6 \\
\bottomrule
\end{tabular}
    \caption{all argument results for the Lung \& Ovarian source}
    \label{table:results_all_arguments_lungovarian}
\end{table}

==> table/results_infrequent_all.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[!ht]
    \centering
\begin{tabular}{lllllll}
\toprule
               &                 &       Full test &    \begin{tabular}[c]{c}  Remove \\      top 20    \end{tabular}   &   \begin{tabular}[c]{c}  Remove \\      top 40    \end{tabular} &   \begin{tabular}[c]{c}  Remove \\      top 60    \end{tabular} &   \begin{tabular}[c]{c}  Remove \\      top 80    \end{tabular} \\
Source & Version &                 &                  &                 &                 &                 \\
\midrule
Covid & Baseline &            77.2 &             66.2 &            61.3 &            59.4 &            56.7 \\
               &      w/ Masking &          78.5** &           68.3** &           63.2* &           61.4* &           58.4* \\
               & + Adaptive Pretraining &            78.6 &             67.9 &            63.5 &            61.7 &            59.4 \\
               &      w/ Masking &  \textbf{80.0*} &  \textbf{70.3**} &  \textbf{65.8*} &  \textbf{64.2*} &  \textbf{61.6*} \\
Lung \& Ovarian & Baseline &            79.2 &             68.0 &            65.3 &            61.3 &            58.9 \\
               &      w/ Masking &          78.2- - &             67.5 &            64.6 &            60.4 &            58.4 \\
               & + Adaptive Pretraining &   \textbf{79.4} &             68.5 &            66.0 &   \textbf{62.5} &            60.4 \\
               &      w/ Masking &            79.2 &    \textbf{68.8} &   \textbf{66.2} &            62.4 &   \textbf{60.6} \\
\bottomrule
\end{tabular}

    \caption{Here are the cross domain results from lung to post on less frequent symptoms after ignoring the top K frequent symptoms from the source training data. To examine the effect of dynamic masking, we use (*) to indicate a p-value below 0.05 and (**) to indicate a p-value below 0.01}
    \label{table:results_infrequent_all}
\end{table}

==> table/results_infrequent_covid.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[!ht]
    \centering
    
\begin{tabular}{|l|l|l|l|}
\hline
                 & removing top-20 & removing top-40 & removing top-60 \\
\hline
Bio-Clinical BERT        & 66.0            & 60.6            & 59.5            \\
+ Dynamic Masking  & 68.8 **         & 64.2 **         & 63.4 **         \\
\hline
DAPT (target-relevant)     & 67.7            & 62.7            & 61.7            \\
+ Dynamic Masking           & \textbf{69.7 *} & \textbf{65.5} **         & \textbf{64.7} ** \\
\hline
\end{tabular}


    \caption{Here are the cross domain results from covid to post on less frequent symptoms after ignoring the top K frequent symptoms from the source training data. To examine the effect of dynamic masking, we use (*) to indicate a p-value below 0.05 and (**) to indicate a p-value below 0.01, similar to Table ~\ref{table:main_results}}
    \label{table:results_infrequent_covid}
\end{table}



==> table/results_infrequent_lung.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}[!ht]
    \centering
\begin{tabular}{|l|l|l|l|}
\hline
                     & removing top-20 & removing top-40 & removing top-60 \\
                     \hline
Bio-Clinical BERT            & 70.7            & 63.2            & 61.0            \\
+ Dynamic Masking              & 70.2            & 63.0            & 61.3            \\
\hline
DAPT (target-relevant) & 71.6   & \textbf{65.2}   & \textbf{63.2}            \\
+ Dynamic Masking               &  \textbf{72.0} 
& 64.7   & 63.1     \\
\hline
\end{tabular}

    \caption{Here are the cross domain results from lung to post on less frequent symptoms after ignoring the top K frequent symptoms from the source training data. To examine the effect of dynamic masking, we use (*) to indicate a p-value below 0.05 and (**) to indicate a p-value below 0.01, similar to Table ~\ref{table:main_results}}
    \label{table:results_infrequent_lung}
\end{table}
